Context-Sensitive and Duration-Aware Qubit Mapping for Various NISQ Devices

Quantum computing (QC) technologies have reached a second renaissance in the last decade. Some fully programmable QC devices have been built based on superconducting or ion trap technologies. Although different quantum technologies have their own parameter indicators, QC devices in the NISQ era share common features and challenges such as limited qubits and connectivity, short coherence time and high gate error rates. Quantum programs written by programmers could hardly run on real hardware directly since two-qubit gates are usually allowed on few pairs of qubits. Therefore, quantum computing compilers must resolve the mapping problem and transform original programs to fit the hardware limitation. To address the issues mentioned above, we summarize different quantum technologies and abstractly define Quantum Abstract Machine (QAM); then propose a COntext-sensitive and Duration-Aware Remapping algorithm (Codar) based on the QAM. By introducing lock for each qubit, Codar is aware of gate duration difference and program context, which bring it abilities to extract more program's parallelism and reduce program execution time. Compared to the best-known algorithm, Codar halves the total execution time of several quantum algorithms and cut down 17.5% - 19.4% total execution time on average in different architectures.

==> concl.tex <==
\section{Conclusion}
\label{sec:concl}
In NISQ era, most quantum programs are not directly executable 
because two-qubit gates can be applied between arbitrary two logical qubits 
while it can only be implemented between two adjacent physical qubits due to hardware constraints. 
To solve this problem,
in this paper we propose \name that can transform the origin circuit and insert necessary \kn{SWAP} operations 
making the circuit comply with the hardware constraints. 
With the design of qubit lock and commutativity detection, 
\mysys is aware of program context and the gate duration difference 
which help \name find the remapping with good parallelism and 
reduce QC's weighted depth. 
Experimental results show that 
compared to the best known remapping algorithm, 
\name can cut down 15.3\% $\sim$ 18.9\% weighted depth at average. 
Using heuristic search, 
\name can find the remapping in a short time and has the ability to fit with large-scale quantum device 
which is necessary in NISQ era.
